TensorFlow: Large-Scale Machine Learning on Heterogeneous Distributed Systems

TensorFlow is an interface for expressing machine learning algorithms, and an implementation for executing such algorithms. A computation expressed using TensorFlow can be executed with little or no change on a wide variety of heterogeneous systems, ranging from mobile devices such as phones and tablets up to large-scale distributed systems of hundreds of machines and thousands of computational devices such as GPU cards. The system is flexible and can be used to express a wide variety of algorithms, including training and inference algorithms for deep neural network models, and it has been used for conducting research and for deploying machine learning systems into production across more than a dozen areas of computer science and other fields, including speech recognition, computer vision, robotics, information retrieval, natural language processing, geographic information extraction, and computational drug discovery. This paper describes the TensorFlow interface and an implementation of that interface that we have built at Google. The TensorFlow API and a reference implementation were released as an open-source package under the Apache 2.0 license in November, 2015 and are available at www.tensorflow.org.

==> Makefile <==
# Makefile for processing tensorflow.tex
#
# % make                # Builds paper.dvi, paper.ps
# % make clean          # Gets rid of all generated files
# % make spell		# Run ispell

default: tensorflow.pdf
all: tensorflow.pdf

# Add any included TeX files to TEXT
STYS = sigmod.sty usenix.sty drafthead.sty macros.sty leftmath.sty toappear.sty
TEXT = $(wildcard *.tex)
TEXS = $(TEXT) $(STYS)

DIAGRAMS = \
  DeviceBoundaries.pdf \
  FeedFetch.pdf \
  ModelParallel.pdf \
  ProcessCloud.pdf \
  SimpleGraph.pdf \
  SyncAsync.pdf \



FIGS =

LDIRT = *.gps *.eps *.lof *.lot *.blg *.toc
DIRT = *.o core *.aux *.dvi *.log *.stamp *.stampold *.i *.bbl *.[ib]lg\
	*.cc.tex *.out $(LDIRT)
GENERATED =
RM = rm -f
DVIPS = dvips
DVIPSOPTS = -P cmz -t letter
TEXSTAMP = ./texstamp
LATEX = latex
JGRAPH = /home/sanjay/bin/i686/jgraph
GRIND = /home/sanjay/bin/i686/grind

.SUFFIXES: .tex .dvi .ps .aux .txt .ind .idx .bbl .aux .jgr .gps .fig .eps .dot

#tensorflow.pdf: tensorflow.ps
#	ps2pdf14 $<

tensorflow.pdf: tensorflow.tex $(FIGS) $(DIAGRAMS) tensorflow.bib $(STYS) $(TEXT)
	pdflatex tensorflow
	bibtex tensorflow
	pdflatex tensorflow.tex
	pdflatex tensorflow.tex

#tensorflow.ps: tensorflow.dvi $(FIGS)
#	$(DVIPS) $(DVIPSOPTS) $< -o $@

#tensorflow.dvi: tensorflow.tex $(FIGS) $(DIAGRAMS) tensorflow.bib $(STYS) $(TEXT)
#	latex tensorflow
#	bibtex tensorflow
#	latex tensorflow
#	latex tensorflow

html:
	latex2html -split 0 -white -no_navigation -info "" -address "" \
	-show_section_numbers \
	tensorflow.tex

pictures: $(FIGS)

spell:
	ispell $(TEXT)

$(FIGS): style.jgr

.dot.eps:
	dot -Tps $< > $@

.jgr.gps:
	$(JGRAPH) $< > $@

.fig.eps:
	fig2dev -L eps $< $@

# Other rules
clean:
	$(RM) $(DIRT)

